Self-learn to Explain Siamese Networks Robustly

Learning to compare two objects are essential in applications, such as digital forensics, face recognition, and brain network analysis, especially when labeled data is scarce and imbalanced. As these applications make high-stake decisions and involve societal values like fairness and transparency, it is critical to explain the learned models. We aim to study post-hoc explanations of Siamese networks (SN) widely used in learning to compare. We characterize the instability of gradient-based explanations due to the additional compared object in SN, in contrast to architectures with a single input instance. We propose an optimization framework that derives global invariance from unlabeled data using self-learning to promote the stability of local explanations tailored for specific query-reference pairs. The optimization problems can be solved using gradient descent-ascent (GDA) for constrained optimization, or SGD for KL-divergence regularized unconstrained optimization, with convergence proofs, especially when the objective functions are nonconvex due to the Siamese architecture. Quantitative results and case studies on tabular and graph data from neuroscience and chemical engineering show that the framework respects the self-learned invariance while robustly optimizing the faithfulness and simplicity of the explanation. We further demonstrate the convergence of GDA experimentally.

==> analysis_old.tex <==
\section{Convergene analysis}
\label{sec:analysis}
We analyze the conditions under which Algorithm~\ref{alg:con_opt} will converge.
Convergence of algorithms for constrained optimization has been studied in~\cite{Seung2007}, from which we adopt their analysis based on dynamical system perspective to provide a proof.
Note that we do not provide a convergence rate in this work. 
We focus on the case when the loss function $\ell$ is convex in the single parameter $\mathbf{m}$ as in Eq. (\ref{eq:con_lm_tabular_obj}).
This excludes the cases when two inputs are having separate masks, for example, when two local masks are learned for two vector or graph inputs.

The Lagrangian function of the optimization problem in Eq. (\ref{eq:con_lm_tabular_obj}) and (\ref{eq:con_lm_tabular_con}) is denoted by $\mathcal{L}(\mathbf{m}, \boldsymbol{\lambda})$ as in Eq. (\ref{eq:lagrangian}).
We prove that the gradient descent-ascent algorithm converges to some stationary point.

\begin{definition}[Stationary points]
A stationary point of $\mathcal{L}(\mathbf{m}, \boldsymbol{\lambda})$ is $(\mathbf{m}^\ast, \boldsymbol{\lambda}^\ast)$ if both
\begin{equation}
     \frac{\partial \mathcal{L}}{\partial \mathbf{m}}(\mathbf{m}^\ast, \boldsymbol{\lambda}^\ast) = \mathbf{0}
     \hspace{.1in}\textnormal{and} \hspace{.1in}
     \frac{\partial \mathcal{L}}{\partial \bl}(\mathbf{m}^\ast, \boldsymbol{\lambda}^\ast) = \mathbf{0}.
\end{equation}
\end{definition}

A stationary $\mathbf{m}^\ast$ may not be a global optimal $\mathbf{m}$ of the constrained optimization problem.
A saddle point is a stationary point so that
\begin{equation}
    \mathcal{L}(\mathbf{m}^\ast, \boldsymbol{\lambda})
    \leq
    \mathcal{L}(\mathbf{m}^\ast, \boldsymbol{\lambda}^\ast)
    \leq
    \mathcal{L}(\mathbf{m}, \boldsymbol{\lambda}^\ast),
    \hspace{.in}
    \forall \boldsymbol{\lambda}, \mathbf{m}.
\end{equation}
In game theory, a saddle point is also called an equilibrium of the min-max game with $\mathcal{L}(\mathbf{m}, \boldsymbol{\lambda}) $ as the payoff function,
where neither player wants to move away from the saddle point.
The convergence analysis only guarantees the convergence of the gradient descent-ascent to a stationary point, which may not be a saddle point.

In a dynamical system, one can regard the movement of a particle with coordinates $(\mathbf{m}(t), \boldsymbol{\lambda}(t))$, which are functions of the time $t$.
The gradient descent-ascent algorithm moves the particle using
\begin{equation}
    \bm(t+1) = \bm(t) - \eta_1\frac{\partial \mathcal{L}}{\partial \bm},\hspace{.1in}
    \bl(t+1) = \bl(t) + \eta_2\frac{\partial \mathcal{L}}{\partial \bl}.
\end{equation}
The update is a discrete approximation of the continuous-time trajectory of the particle, so that the infinitestimal movement of the particle can be calculated by the derivative of the trajectory w.r.t. the time variable $t$:
\begin{equation}
\label{eq:gda_dynamics}
    \dot{\bm} \triangleq \frac{d \bm(t)}{dt}=-\frac{\partial \mathcal{L}}{\partial \bm},
    \hspace{.1in}
    \dot{\bl} \triangleq \frac{d \bl(t)}{dt}=\frac{\partial \mathcal{L}}{\partial \bl}.
\end{equation}

We construct a Lyapunov function $V:\mathbb{R}^n\to \mathbb{R}$ as follows:
\begin{equation}
    V(\bm,\bl) = \frac{1}{2}\|\dot{\bm}\|_2^2
    + \frac{1}{2}\|\dot{\bl}\|_2^2
    - r \mathcal{L}(\bm, \bl).
\end{equation}
$r$ should be chosen so that $V$ is strictly positive and can be interpreted as an energy function (the kinetic energy $\frac{1}{2}\|\dot{\bm}\|_2^2
    + \frac{1}{2}\|\dot{\bl}\|_2^2$
    plus the potential energy $-r\mathcal{L}(\bm, \bl)$).
The energy is a function of $t$ as both its arguments are,
and the convergence of the dynamics $\dot{\bm}$ and $\dot{\bl}$ can be proved by showing that the energy converges to 0 as $t\to\infty$.
By taking the derivative of $V$ w.r.t. $t$, we find that the necessary condition for $V$ to converge to $0$ is when the following matrix is positive definite:
\begin{equation}
    \left[
    \begin{array}{cc}
        \mathcal{L}_{\bm\bm}-rI, & 0\\
        0, &  rI-\mathcal{L}_{\bl\bl}
    \end{array}
    \right]
    \triangleq
    \left[
    \begin{array}{cc}
        \frac{\partial^2\mathcal{L}}{\partial \bm^2}, & 0\\
        0, & \frac{\partial^2\mathcal{L}}{\partial \bl^2}
    \end{array}
    \right]
\end{equation}

We rephrase Theorem 1 from~\cite{Seung2007} as follows.
\begin{theorem}
Suppose that the stationary points of the gradient descent-ascent dynamics Eq. (\ref{eq:gda_dynamics}) are isolated, and
\begin{equation}
    \lambda_{\textnormal{inf}}(\mathcal{L}_{\bl\bl})\triangleq\sup_{\bm, \bl} \lambda_{\textnormal{max}} (\mathcal{L}_{\bl\bl})
    <
    \inf_{\bm, \bl} \lambda_{\textnormal{min}} (\mathcal{L}_{\bm\bm})
    \triangleq\lambda_{\textnormal{inf}}(\mathcal{L}_{\bm\bm}).
\end{equation}
Then any bounded trajectory converges to a stationary point.
\end{theorem}
% According to the theorem, we don't requires the Lagrangian to be convex in the argument $\bm$ and concave in the argument $\bl$, but need the Lagrangian to be ``more convex in $\bm$ than in $\bl$'', or be ``more concave in $\bl$ than in $\bm$''.
Since the Lagrangian $\mathcal{L}(\bm, \bl)$ is linear in $\bl$, $\lambda_{\textnormal{max}} (\bl\bl)=0$.
% We just need to prove that the Hessian matrix $\mathcal{L}_{\bm\bm}$ is positive definite.
As a result, convergence of the gradient descent-ascent is not guaranteed to converge when the faithfulness loss function is not strictly convex.
This is not true for all Siamese network architecture in general, but in the special case when the objective function Eq. (\ref{eq:con_lm_tabular_obj}) is convex,
including the case when
\begin{equation}
\ell\left(f(\mathbf{m} \otimes \mathbf{x}^s, \mathbf{m} \otimes \mathbf{x}^t)
    \right) =\sigma(\left<\mathbf{m} \otimes \mathbf{x}^s, \mathbf{m} \otimes \mathbf{x}^t\right>).
\end{equation}

It remains to prove that any trajectories of gradient descent-ascent is bounded.
\begin{definition}{Radially boundedness}
A function $f(\mathbf{x})$ is radially bounded if $f(\mathbf{x})\to \infty$ if $\|\mathbf{x}\|\to \infty$.
\end{definition}

We use Theorem 2 from~\cite{Seung2007} to make the claim.
\begin{theorem}
    Suppose that $\lambda_{\textnormal{sup}}(\mathcal{L}_{\bl\bl})<\lambda_{\textnormal{inf}}(\mathcal{L}_{\bm\bm})$.
    If $\lambda_{\textnormal{inf}}(\mathcal{L}_{\bm\bm})>0$ and
    the dual objective function $-\min_{\bm}\mathcal{L}(\bm, \bl)$ is radially unbounded,
    then any trajectory of gradient descent-ascent is bounded.
\end{theorem}
It is hard to find the dual objective function in closed-form to directly verify its radial boundedness,
but we can still prove that as $\|\bl\|\to\infty$,
$-\min_{\bm}\mathcal{L}(\bm, \bl)\to \infty$.
It is safe to assume that there is at least one $\lambda_i\neq 0$, so that we can make $m_i\to -\infty$ and $\lambda_i(m_i - M_i)\to -\infty$ as $M_i$ is a given constant in the optimization problem.


==> diversity.tex <==


\subsection{Diversity evaluation}
\begin{table}[]
    \footnotesize
    \centering
    \caption{\small Performance (mean $\pm$ std.) of each algorithm in terms of \textit{diversity} in tabular data by three metrics, \textit{Jaccard similarity}, \textit{Hamming distance} and \textit{Cosine distance}.
    $\mathcal{D}$ in Eq. (\ref{eq:metric_diversity}) includes all compared references for each query.
    The methods with the least diversity are in bold.}
    \label{tab:diversity}
    \begin{tabular}{c || c c c c c}
        \toprule
        \textbf{Metrics} &
        \textbf{Dataset} & SNX-KL & SNX-UC & SNX-DES 
        & SNX \\
        \midrule
        \multirow{4}{*}{\textbf{Jaccard}} 
        & Adult & \textbf{0.57} $\pm$ 0.18 & 0.55 $\pm$ 0.20 & 0.51 $\pm$ 0.18 
        & 0.51 $\pm$ 0.17 \\
        & Bank & 0.64 $\pm$ 0.14 & 0.53  $\pm$ 0.15 & 0.63 $\pm$ 0.14 
        & \textbf{0.65} $\pm$ 0.15 \\
        & Credit & 0.45 $\pm$ 0.16 & 0.42 $\pm$ 0.14 & 0.49 $\pm$ 0.18
        & \textbf{0.59} $\pm$ 0.19 \\
        & COMPAS & \textbf{0.67} $\pm$ 0.18 & 0.79 $\pm$ 0.11 & 0.68 $\pm$ 0.14
        & 0.74 $\pm$ 0.13 \\
        \midrule
        \multirow{4}{*}{\textbf{Hamming}} 
        & Adult & \textbf{5.74} $\pm$ 2.88 & 6.24 $\pm$ 3.56 & 6.89 $\pm$ 3.10 
        & 6.83 $\pm$ 3.00 \\
        & Bank & 4.51 $\pm$ 2.09 & 6.46 $\pm$ 2.48 & 4.68  $\pm$ 2.20
        & \textbf{4.39} $\pm$ 2.16 \\
        & Credit & 7.88 $\pm$ 3.04 & 8.42 $\pm$ 2.69 & 7.18 $\pm$ 3.25 
        & \textbf{7.08} $\pm$ 3.42 \\
        & COMPAS & 4.24 $\pm$ 2.61 & \textbf{2.42} $\pm$ 1.33 & 3.96 $\pm$ 2.07 
        & 3.13 $\pm$ 1.84 \\
        \midrule
        \multirow{4}{*}{\textbf{Cosine}} 
        & Adult & \textbf{0.29} $\pm$ 0.14 & 0.31 $\pm$ 0.18 & 0.34 $\pm$ 0.16 
        & 0.34 $\pm$ 0.15 \\
        & Bank & 0.23 $\pm$ 0.10 & 0.32 $\pm$ 0.12 & 0.23 $\pm$ 0.11 
        & \textbf{0.22} $\pm$ 0.11 \\
        & Credit & 0.39 $\pm$ 0.15 & 0.42 $\pm$ 0.13 & 0.36 $\pm$ 0.16 
        & \textbf{0.35} $\pm$ 0.17 \\
        & COMPAS & 0.21 $\pm$ 0.13 & \textbf{0.12} $\pm$ 0.07 & 0.20 $\pm$ 0.10 
        & 0.16 $\pm$ 0.09 \\
        \bottomrule
    \end{tabular}
\end{table}


\textit{Diversity} of explanations have been proposed as a metric when there are multiple feasible (counterfactual) explanations~\cite{mothilal2020explaining,Russell2019}.
We study the diversity of the set of masks  $\mathbf{m}^s$ extracted from $\mathbf{x}^s$ when $\mathbf{x}^s$ is compared with different references $\mathbf{x}^t$.
Generally, $\mathbf{x}^s$ should depend on both input instances $\mathbf{x}^s$ and $\mathbf{x}^t$, namely, $\mathbf{m}^s = \mathbf{m}^s(\mathbf{x}^s, \mathbf{x}^t)$,
and we have the following diversity metric:
\begin{equation}
\label{eq:metric_diversity}
    \sum_{\mathbf{x}^t, \Tilde{\mathbf{x}}^t \in \mathcal{D}}
    dist \left( 
    \mathbf{m}^s(\mathbf{x}^s,\mathbf{x}^t), 
    \mathbf{m}^s(\mathbf{x}^s, \Tilde{\mathbf{x}}^t) \right),
\end{equation}
where $dist$ can be one minus cosine/Jaccard similarity or Hamming distance on tabular data, or Graph Edit Distance~\cite{Sanfeliu83} on graph data.
$\mathcal{D}$ includes all references compared with $\mathbf{x}^s$.
% for example,
% $\mathcal{D}$ can contain all same-class references as one query's.
A high diversity score indicates the set of masks $\mathbf{m}^s$ vary a lot along with the references.
The approach in~\cite{utkin2019explanation} extracts salient features of $\mathbf{x}^s$ without concerning the references, namely, 
$\mathbf{m}^s = \mathbf{m}^s(\mathbf{x}^s)$,
and there is no diversity.
While prior work advocates high diversity~\cite{Russell2019}, a high explanation diversity is desirable only when it is highly faithful.

% \begin{table}[h]
%     \centering
%     \caption{\small Performance (mean $\pm$ std.) of each algorithm in terms of \textit{diversity} in tabular data by Jaccard distance, 
%     $\mathcal{D}$ in Eq. (\ref{eq:metric_diversity}) includes all compared references for each query.
%     %%%%% Experimental settings to obtain the results %%%%%
%     %
%     % Settings: we evaluate the diversity by Jaccard distance.
%     % We first filter out all references being compared to a query, 
%     % then compute the Jaccard distance of each pair within them.
%     % For example, if a query is compared with other 4 references, 
%     % we need to evaluate distance between 4*3/2 = 6 pairs.
%     % Then, we compute diversity for each query, and aggregate these numbers for a mean and standard deviation.
%     % A value being closer to 1 indicates the method generates less diverse masks when comparing with different references.
%     % 
%     %%%%%%%%%%% 
%     }
%     \footnotesize
%     \begin{tabular}{c c c c c c}
%         \toprule
%         \textbf{Dataset} & KL-soft & Unconstrained & DES-local 
%         % & XX-inter & XX-union 
%         & XX \\
%         \midrule
%         Adult & 0.57 $\pm$ 0.18 & 0.55 $\pm$ 0.20 & 0.51 $\pm$ 0.18 
%         & 0.51 $\pm$ 0.17 \\
%         Bank & 0.64 $\pm$ 0.14 & 0.53  $\pm$ 0.15 & 0.63 $\pm$ 0.14 
%         & 0.65 $\pm$ 0.15 \\
%         Credit & 0.45 $\pm$ 0.16 & 0.42 $\pm$ 0.14 & 0.49 $\pm$ 0.18
%         & 0.59 $\pm$ 0.19 \\
%         COMPAS & 0.67 $\pm$ 0.18 & 0.79 $\pm$ 0.11 & 0.68 $\pm$ 0.14
%         & 0.74 $\pm$ 0.13 \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:diversity}
% \end{table}
\vspace{.1in}
\noindent\textbf{Do the reference-specific masks have diversity?}
\textcolor{red}{Diversity should be shorten.}
Table~\ref{tab:diversity} shows diversity of the local masks evaluated in three distance metrics, Jaccard similarity, cosine similarity and Hamming distance.
% One may expect that multiple reference-specific masks $\mathbf{m}^s$ for the same query will have little diversity under the constraints of the same global invariant mask $\mathbf{M}^s$.
% However, 
% As Table \ref{tab:diversity} shows,
We can see that SNX has 
the largest diversity on the Bank and Credit dataset and is the runner-up on the COMPAS dataset.
Given the faithfulness performance in Table \ref{tab:overall}, and the percentage of constraints violated shown in Figure~\ref{fig:kl-lag},
we conclude that the global masks is sufficiently flexible for the local masks to fit different references $\mathbf{x}^t$, leading to
both high diversity and faithfulness.
On the contrary,
stage 2 optimization without constraint has the lowest diversity on the Bank and Credit datasets.
Given that \textit{Unconstrained} is outperformed by XX in faithfulness in Table~\ref{tab:overall}, we conclude that this baseline focuses on a smaller set of less salient features.
\textcolor{red}{Need to combine the evidence about constraint violation in this discussion.}

==> method-copy.tex <==
\section{Methodology}
\label{sec:methodology}
We propose optimization problems and a gradient descent-ascent algorithm to generate explanations. 
% with a convergence guarantee. 
% Convergence of the algorithm is in the next section.

\subsection{General Formulation}
\label{sec:general_opt}
The variables to be optimized are the two masks $\mathbf{m}^s \in [0,1]^{p_s}$ and $\mathbf{m}^t \in [0,1]^{p_t}$ over query $\mathbf{x}^s$ and reference $\mathbf{x}^t$, respectively
\footnote{The sigmoid function 
% $\sigma(\cdot)$ 
squashes each real-valued mask element to $[0,1]$.}.
% two masks on $\mathbf{x}^s$ and $\mathbf{x}^t$.
% To ensure all elements in masks are in [0,1], 
% we apply the sigmoid function, $\sigma(\cdot)$, to all masks.
% but drop it in the optimization formulations for the simplicity.
To balance the faithfulness and simplicity,
% need to be simple and faithful, 
we have the objective:
\begin{equation}
    \min_{\mathbf{m}^s, \mathbf{m}^t}  
    \ell \left( 
    f(\mathbf{x}^s, \mathbf{x}^t),
    f(\mathbf{m}^s \otimes \mathbf{x}^s, 
    \mathbf{m}^t \otimes \mathbf{x}^t) \right) 
    +\gamma(\| \mathbf{m}^s \| + \| \mathbf{m}^t \|),\label{eq:obj_lm}
\end{equation}
where
$\gamma $ is a hyperparameter to fine-tune the relative importance of the two goals.
$\ell(\cdot,\cdot)$ as defined by Eq. (\ref{eq:faith}) promotes faithfulness
and $\|\cdot\|$ is the $\ell_1$-norm that promotes simplicity.
% which do not consider the compared objects.
% Besides,
% $\mathbf{m}^s$ and $\mathbf{m}^t$ have the same dimension as $\mathbf{x}^s$ and $\mathbf{x}^t$, respectively,
% and thus can have different dimensions for two different graphs input to the SN model.
%
% On the one hand,
% if $\mathbf{m}^s$ is a function of both $\mathbf{x}^s$ and $\mathbf{x}^t$,
% % $\mathbf{m}^s$ can be significantly influenced by $\mathbf{x}^t$.
% when $\mathbf{m}^s$ is compared with $\tilde{\mathbf{x}}^{t}$ that is dramatically different from $\mathbf{x}^{t}$,
% $\mathbf{m}^s$ can be changed to $\tilde{\mathbf{m}}^{s}$ that is not much related to $\mathbf{m}^s$.
% It is hard for humans to connect $\mathbf{m}^{s}$ to $\tilde{\mathbf{m}}^{s}$ when they are expected to retain invariance in the same query.
% On the other hand, making $\mathbf{m}^{s}$ independent of $\mathbf{x}^t$ provides no flexibility and can't faithfully explain the distinct behaviors of the SN when comparing $\mathbf{x}^s$ with different references.
% According to the robustness characterization,
The mask $\mathbf{m}^s$ is a function of $\mathbf{m}^t\otimes\mathbf{x}^t$ and can lack robustness if a saliency map is adopted.
We use a global invariant to regulate $\mathbf{m}^s$ for more robustness against varying 
% references 
$\mathbf{m}^t$.
% We formulate a two-stage optimization framework to adaptively balance such invariance and flexibility.

\vspace{.1in}
\noindent\textbf{Stage 1}.
If there is domain knowledge regarding which features/edges in an instance $\mathbf{x}$ are salient,
or sensitive features prohibited due to fairness requirement,
we can set the corresponding mask values to 1 or 0 
accordingly 
in a global mask $\mathbf{M}$ for $\mathbf{x}$.
If there is no such knowledge,
we propose to extract $\mathbf{M}$ 
% for $\mathbf{x}$ 
to provide globally invariant properties in $\mathbf{x}$ regardless of references,
% any reference instances,
using the 
% following
self-supervision learning problem:
% where the faithfulness of $\mathbf{M}$ is evaluated by Eq. (\ref{eq:faith}) as well.
% Therefore we propose the following optimization problem to extract a global mask $\mathbf{M}$ for each input
% (either $\mathbf{M}^s$ for query $\mathbf{x}^s$ or $\mathbf{M}^t$ for reference $\mathbf{x}^t$)
% that fits the SN.
\begin{equation}
\label{eq:obj_gm}
    \min_{\mathbf{M}\in[0,1]^p} 
    \ell \left(
    f(\mathbf{x}, \mathbf{x}),
    f(\mathbf{x}, \mathbf{M} \otimes \mathbf{x})
    \right) 
    + \gamma \| \mathbf{M} \|.
\end{equation}
% where we use the Binary Cross Entropy as the distance measurement $\ell(\cdot,\cdot)$ as before.
$\mathbf{M}$ is expected to extract the salient features of $\mathbf{x}$ to maximally preserve information in $\mathbf{x}$, indicated by a low faithfulness loss when comparing $\mathbf{x}$ and $\mathbf{M} \otimes \mathbf{x}$.
% It is important to consider the target SN $f$ when finding $\mathbf{M}$.
Unsupervised feature selection~\cite{wei2017rethinking} can learn important features but does not consider the target SN,
and usually fails in sanity check \cite{adebayo2018sanity}.
% This alternative is also not applicable to graph data.
% We empirically compare the global mask $\mathbf{M}$ with features selected by the unsupervised selection algorithm in \cite{wei2017rethinking} in Sec \ref{sec:exp_global_mask}.
% \textit{Besides, we do not utilize unsupervised feature selection for the purpose that the global mask is tied to the parameters of the SN.}


% \subsection{Connection to Self-learning}
% Consider the self-learning loss in self-learning consists of two parts, one for domain task and one for self-learning \cite{you2020graph},
% where self-learning loss $\mathcal{L}_{self}$ is derived from multiple types of transformations on both node/edge level and graph level \cite{you2020graph,jin2020self}.
\textit{Connection to Self-Supervised Learning (SSL).}
Multiple types of transformations on both node/edge level and graph level are proposed in SSL \cite{you2020graph,jin2020self}.
For example, 
based on the assumption that subgraphs can indicate the full graphs' semantics in \cite{jin2020self},
the embedding of the subgraphs generated by random walk should be similar to the embedding of the original graphs.
The objective function in SSL can be:
\begin{equation*}
f^\ast 
= \min_f \mathcal{L}_{self} (\mathbf{M}, \mathbf{x}, f) 
= \min_f \ell (f(\mathbf{x}), f(\mathbf{M} \otimes \mathbf{x} ) ),
\end{equation*}
where $\ell$ is a temperature cross entropy and $\mathbf{M}$ is subgraph transformation generated by random walk in \cite{jin2020self}.
Comparing the objective function with Eq. (\ref{eq:obj_gm}),
the key difference is that the variables in SSL to optimize are parameters of the model, 
while we focus on the transformation (extracting subgraphs).
% two key differences can be addressed:
% a) the variables in SSL to optimize are parameters of the model, 
% % $\min_f \mathcal{L}_{self}(\mathbf{M}, \mathbf{x}, f)$; 
% while we focus on the transformation (extracting subgraphs),
% % $\min_\mathbf{M} \mathcal{L}_{self}(\mathbf{M}, \mathbf{x}, f)$,
% % with a fixed model $f$,
% and
% b) models $f$ in SSL accept single input \cite{jin2020self,you2020graph}, 
% while our method consider SN with two inputs.



\vspace{.1in}
\noindent\textbf{Stage 2}.
We incorporate the global masks $\mathbf{M}^s$ and $\mathbf{M}^t$ as constraints to the optimization problem Eq. (\ref{eq:obj_lm}) to find local masks $\mathbf{m}^s$ and $\mathbf{m}^t$:
% \begin{equation}
\begin{align}
% \arraycolsep=1.4pt\def\arraystretch{1.5}
    % \begin{array}{cc}
    \min_{\mathbf{m}^s, \mathbf{m}^t} & 
    \ell \left( 
    f(\mathbf{x}^s, \mathbf{x}^t),
    f(\mathbf{m}^s \otimes \mathbf{x}^s, 
    \mathbf{m}^t \otimes \mathbf{x}^t)
    \right) 
    + \gamma \left(\| \mathbf{m}^s \| + \| \mathbf{m}^t \| \right),\label{eq:con_lm_obj} \\
    \textnormal{s.t.} 
    & \quad
    g_i(\mathbf{m}) =\mathbf{m}^s_i - \mathbf{M}^s_i \leq 0, 
    \: \forall i \in \{1, \dots, p_s\},\label{eq:con_lm_con_1}\\
    & \quad 
    g_{p_s+i}(\mathbf{m}) = \mathbf{m}^t_i - \mathbf{M}^t_i \leq 0, 
    \: \forall i \in \{1, \dots,  p_t \}\label{eq:con_lm_con_2}.
\end{align}
% \end{equation}
% \begin{align} 
% x_{\rm L} & = L \int{\cos\theta\left(\xi\right) d\xi}, \label{eq_1} \\\\
% y_{\rm L} & = L \int{\sin\theta\left(\xi\right) d\xi}, \nonumber
% \end{align}
% \end{eqnarray}
The constraints require local masks $\mathbf{m}^s$ and $\mathbf{m}^t$ to be element-wise no greater than the corresponding global masks $\mathbf{M}^s$ and $\mathbf{M}^t$, which reduce the freedom in choosing $\mathbf{m}^s$ and $\mathbf{m}^t$.
% \footnote{$\mathbf{m}_i \leq \mathbf{M}_i$ is equivalent to $\sigma(\mathbf{m}_i)  \leq \sigma(\mathbf{M}_i)$ for the monotonicity of the sigmoid function.}
% The optimization problem can further incorporate slack variables for each
However, the optimization algorithm allows some violations of the constraints, so that the local masks have the flexibility to go beyond the global masks to adapt to different references.
% More generally, the global masks can be used to specify constraints from domain experts.
% For example, when a clinical researchers is wondering if the target SN distinguishes a bipolar subject from healthy controls using a known brain network connection pattern, the global mask can be set to allow all local explanations for the subject to select this pattern.
% In other words,
% the global masks $\mathbf{M}$ extract global invariant features for each instance, 
% which find more fine-grained salient features when comparing a specific pair of query and reference.
% \textcolor{red}{The stabilizing effect of global masks on the local masks will be validated by human experiments (see Section \ref{sec:human_validation}).}
% The above optimization problems will next be specified to tabular data (Section. \ref{sec:opt_tabular}) and graph data (Section \ref{sec:opt_graph}).

% \begin{table*}[]
%     % \centering
%     \begin{tabular}{cc||c|c|c|c|c|c|c|c|c}
%     \multirow{2}{*}{label} &
%     \multirow{2}{*}{$ \gamma $} &
%     \multicolumn{9}{c}{Major Features} \\
%      && Work class & Race & Education & Age
%      & Hours/Week & Marital status & Occupational & Relationship & Sex \\
%      \hline
%      Pos & 1e-4 & 0.71 & 0.75 & 0.79 & 0.47 & 0.70 & 0.74 & 0.78 & 0.79 & 0.43 \\
%      Pos & 1e-3 & 0.56 & 0.63 & 0.65 & 0.35 & 0.58 & 0.60 & 0.69 & 0.66 & 0.34 \\
%      \hline
%      Neg & 1e-4 & 0.18 & 0.26 & 0.67 & 0.42 & 0.40 & 0.48 & 0.60 & 0.56 & 0.37 \\
%      Neg & 1e-3 & 0.06 & 0.08 & 0.43 & 0.21 & 0.23 & 0.28 & 0.45 & 0.36 & 0.08
%     \end{tabular}
%     \caption{
%     \footnotesize
%     After applying Eq. (1) to search mask for \textit{each} sample, the table shows the ratio of global masks picking major features for samples with specific labels and hyperparameters($ \gamma $).}
%     \label{tab:major_features}
% \end{table*}



\subsection{Optimization for tabular data}
\label{sec:opt_tabular}
\noindent \textbf{Stage 1.}
Without a particular reference $\mathbf{x}^t$,
% at stage 1,
a global mask over a query can at best identify salient major features, such as \texttt{Age}, in  $\mathbf{z}^s$.
In stage 2, with $\mathbf{x}^t$,
we can identify salient minor features, such ``\texttt{Age}<25'', associated with the salient major features.
We introduce a global invariant mask $\mathbf{N}\in[0,1]^{q}$ over the major features,
where $\mathbf{N}_{i}$ is the importance of the $i$-th major feature.
Regarding the global mask $\mathbf{M}$ over the minor features,
$\mathbf{M}_{i,j}$ indicates the importance of the $j$-th value of the $i$-th major categorical feature.
% $\mathbf{N}$ are not variables to be optimized directly,
Based on one-hot encoding,
$\mathbf{N}_i = 1 - \prod_j (1-\mathbf{M}_{i,j}), i=1,\dots, q$,
meaning that
if a major feature $z_i$ is salient, then at least one of the associated minor features $x_{i,j}$ needs to be salient too.
We optimize global masks $\mathbf{M}$, with $\mathbf{N}$ as an intermediate variable, as follows:
\begin{eqnarray}
\label{eq:obj_gm_tabular}
    \min_{\mathbf{M}} & \ell \left(
    f(\mathbf{x}, \mathbf{x}),
    f(\mathbf{x}, \mathbf{M} \otimes \mathbf{x}) \right) 
    + \gamma \|\mathbf{N} \|, \\
    \label{eq:obj_gm_tabular_Ni}
    & \textnormal{s.t.} \quad \mathbf{N}_i = 1 - \prod_j (1-\mathbf{M}_{i,j}), 
    \forall i \in \{ 1, \dots, q \}.
\end{eqnarray}
The alternatives $\mathbf{N}_i = \sum_k \mathbf{M}_{i,k}$
scales linearly in the number of minor features for a major feature and the sum can go beyond 1.
In addition, minimizing $ \sum_k \mathbf{M}_{i,k}$ in the $\ell_1$ norm regularization can lead to many small non-zeros in $M_{i,j}$, so that the major feature is significant but none of the associated minor features is.
The option $\mathbf{N}_i =\prod_k \mathbf{M}_{i,k}$ does not work either: it
shrinks to 0 quickly as the number of minor features increases.
% A categorical feature with many possible values will have more minor features selected.
The proposed $\mathbf{N}_i = 1 - \prod_j (1-\mathbf{M}_{i,j})$ selects a similar number of minor features for each major feature.
% In adapting Eq. (\ref{eq:obj_gm}) to learn global masks,,
% For simplicity,
We apply $\ell_1$ regularization to $\mathbf{N}$ rather than to $\mathbf{M}$
% over minor features,
for the same reason that $\mathbf{N}_i = \sum_k \mathbf{M}_{i,k}$ is not adopted.
% On the contrary, minimizing the $\ell_1$ norm of $\mathbf{N}$ directly


\noindent \textbf{Stage 2.}
For tabular data, any two input vectors to SN are aligned,
so we optimize a single mask $\mathbf{m}=\mathbf{m}^s=\mathbf{m}^t$ to find salient features for both instances.
Similar to Eq. (\ref{eq:obj_gm_tabular_Ni}),
we define the local masks over major features as $\mathbf{n}_i = 1 - \prod_j (1-\mathbf{m}_{i,j})$,
and adopt the $\ell_1$ regularization as in Eq. (\ref{eq:obj_gm_tabular}).
\begin{eqnarray}
\label{eq:con_lm_tabular_obj}
    \min_{\mathbf{m}} & \ell \left(
    f(\mathbf{x}^s, \mathbf{x}^t),
    f(\mathbf{m} \otimes \mathbf{x}^s, \mathbf{m} \otimes \mathbf{x}^t)
    \right) 
    + \gamma \|\mathbf{n} \|, \\
    % \label{eq:con_lm_tabular_con}
    &\textnormal{s.t.}  \quad g_i(\mathbf{m}) = \mathbf{n}_i - \mathbf{N}_i \leq 0, 
    \forall i \in \{ 1, \dots, q. \} 
    \label{eq:con_lm_tabular_ineq}\\
    & 
    \quad \quad \mathbf{n}_i = 1 - \prod_j (1- \mathbf{m}_{i,j}), 
    \forall i \in \{ 1, \dots, q\}, \label{eq:con_lm_tabular_mi}\\
    & \quad \quad \mathbf{N}_i = 1 - \prod_j (1- \mathbf{M}_{i,j}), 
    \forall i \in \{ 1, \dots, q \}. \label{eq:con_lm_tabular_Mi}
\end{eqnarray}
% In the above problem,
As we focus on finding related masks for the query $\mathbf{x}^s$ with varying references $\mathbf{x}^t$, we let $\mathbf{M}=\mathbf{M}^s$ (the global invariant mask for $\mathbf{x}^s$) by default, and other variants of $\mathbf{M}$ will be evaluated in the experiments.
% $\mathbf{N}$ in Eq. (\ref{eq:con_lm_tabular_con}) is a constant vector derived from the local mask on the major feature $\mathbf{M}$ optimized in stage 1.
% Eq. (\ref{eq:obj_gm_tabular_Ni}) and Eq. (\ref{eq:con_lm_tabular_ni}) are not ``real" constraints since 
Both $\mathbf{n}$ and $\mathbf{N}$ are not optimization variables, 
but are intermediate variables derived from $\mathbf{m}$ and $\mathbf{M}$, respectively.
% for the $\ell_1$ regularization for sparsity and the inequality constraints for global invariance. 
The $\ell_1$ regularization is placed on the mask $\mathbf{n}$, rather than $\mathbf{m}$, for the same reason analyzed in stage 1.
The inequality constraints over $\mathbf{n}$ balance the invariance from $\mathbf{N}$ and flexibility in $\mathbf{n}$.
Alternatively, the above inequality constraint can be replaced by
a regularization term
%using KL-divergence between the local and global masks $\textnormal{KL}(\mathbf{n}\|\mathbf{N})$:
\begin{equation}
\label{eq:kl_reg}
 \min_{\mathbf{m}} \ell \left(
    f(\mathbf{x}^s, \mathbf{x}^t),
    f(\mathbf{m} \otimes \mathbf{x}^s, \mathbf{m} \otimes \mathbf{x}^t)
    \right) 
    + \gamma \|\mathbf{n} \| 
    + \beta \textnormal{KL}(\mathbf{n} \| \mathbf{N}),
\end{equation}
where 
$\textnormal{KL}(\mathbf{n} \|  \mathbf{N})=\sum_{i=1}^q \textnormal{KL}(\mathbf{n}_i\| \mathbf{N}_i)$ and 
$\textnormal{KL}(\mathbf{n}_i\| \mathbf{N}_i)$ is the KL-divergence between $\mathbf{n}_i$ and $\mathbf{N}_i$, treated as the means of two binary random variables. 
According to~\cite{bishop2006pattern} (Section 10.1),
the KL-regularization encourages $\mathbf{n}_i$ to be smaller than $\mathbf{N}_i$.

% Technical details: the global masks $\mathbf{M}^s$ and $\mathbf{M}^t$ were learned in stage 1 for both the query and the reference, while we are interested in a single local mask $\mathbf{m}$.
% There are several ways to merge $\mathbf{M}^s$ and $\mathbf{M}^t$ into a single mask for Eq. (\ref{eq:con_lm_tabular_Mi}).
% For example, we can set $\mathbf{M} = \min(\mathbf{M}^s, \mathbf{M}^t)$ or $\mathbf{M} = \max (\mathbf{M}^s, \mathbf{M}^t)$ (element-wise min or max), resulting in the symmetry of $\mathbf{m}$ for both the query and reference.
% Alternatively, %following the previous settings in Eq. (\ref{eq:con_lm_con}),
% we can set $\mathbf{M}=\mathbf{M}^s$ if we only care about the global invariance in $\mathbf{x}^s$.
% We will empirically evaluate these alternatives.

% As mentioned in Sec. \ref{sec:data_structure},
% we feed minor features $\mathbf{x}$ into SN,
% and thus we extract masks $\mathbf{M}$ and $\mathbf{m}$ over minor features.
% However,
% highlighting salient features on major level is also interesting for end-users and researchers,
% for example, exploring the key features for decisions.
% Here, we denote global and local masks on major features as $\mathbf{N}$ and $\mathbf{n}$, respectively.
% $\mathbf{M}_{i,j}$ indicates if $\mathbf{M}$ highlights the $j$-th possible value in the $i$-th major feature
% and $\mathbf{N}_{i}$ is the mask on the $i$-th major feature.
% $\mathbf{N}$ and $\mathbf{n}$ are not variables to be optimized directly, 
% but defined by $\mathbf{N}_i \coloneqq 1 - \prod_k (1-\mathbf{M}_{i,k})$ 
% (same for $\mathbf{n}$ by $\mathbf{m}$).
% The intuition is that if a major feature is not part of an explanation, 
% then any of its values, 
% encoded by the corresponding minor features, 
% become irrelevant and can be filtered out.
% We do not use the sum, 
% e.g., $\mathbf{n}_i=\sum_k \mathbf{m}_{i,k}$, 
% because the value of $\mathbf{n}_i$ can be larger than one.
% Another reason is that if the summation over $k$ is large, 
% then $n_i$ can be rather large. 
% In other words, 
% the scale of $n_i$ will depend on the number of possible values that the $i$-th major feature can take.
% % moreover, 
% % $\mathbf{n}_i$ is highly related to the number of corresponding minor features,
% % the more minor features $\mathbf{n}_i$ corresponding to, the higher values $\mathbf{n}_i$ can take.
% Using the product directly,
% e.g., $\mathbf{n}_i = \prod_k \mathbf{m}_{i,k}$,
% results in similar issues,
% which is the more minor features $\mathbf{n}_i$ corresponding to, the lower values $\mathbf{n}_i$ will take due to $\mathbf{m}_{i,k} \in[0,1]$.

% \noindent \textbf{Usage of masks on major features.}
% Revisiting two optimization problems Eq. (\ref{eq:obj_gm}) and Eq. (\ref{eq:con_lm_obj}) with Eq. (\ref{eq:con_lm_con}),
% we propose to apply $\ell_1$-norm and the constraints to the major features rather than minor features for emphasizing the roles of major features.
% Consider the case that $\ell_1$-norm and the constraints on minor features,
% every entry in the minor-level mask will make the same contribution even from different major features,
% which is undesired.
% For example,
% $\mathbf{M}_{i,a}$ and $\mathbf{M}_{j,b}$ taking the same value will make exactly the same contribution for computing $\ell_1$-norm,
% however, their contributions should be related to their corresponding major features.


% \noindent \textbf{Optimization for tabular data.}
% Notice that the meaning of each entry in the feature vectors of the two inputs to the SN are aligned,
% we can simply set $\mathbf{m} = \mathbf{m}^s = \mathbf{m}^t$ to decrease the number of parameters.
% As well as considering the usage of masks on major features,
% we specify the objective functions on the tabular data explicitly:
% \begin{eqnarray}
% \label{eq:obj_gm_tabular}
%     \min_{\mathbf{M}} & \ell \left(
%     f(\mathbf{x}, \mathbf{x}),
%     f(\mathbf{x}, \mathbf{M} \otimes \mathbf{x}) \right) 
%     + \gamma \|\mathbf{N} \|, \\
%     \label{eq:obj_gm_tabular_Ni}
%     & \textnormal{s.t.} \quad \mathbf{N}_i = 1 - \prod_k (1-\mathbf{M}_{i,k}), \forall i.
% \end{eqnarray}
% \begin{eqnarray}
% \label{eq:con_lm_tabular_obj}
%     \min_{\mathbf{m}} & \ell \left(
%     f(\mathbf{x}^s, \mathbf{x}^t),
%     f(\mathbf{m} \otimes \mathbf{x}^s, \mathbf{m} \otimes \mathbf{x}^t)
%     \right) 
%     + \gamma \|\mathbf{n} \|, \\
%     \label{eq:con_lm_tabular_con}
%     & 
%     \textnormal{s.t.} \quad  g_i(\mathbf{m}) \coloneqq \mathbf{n}_i - \mathbf{N}_i \leq 0, \forall i \in 
%     \{1, \dots, q\} \\
%     \label{eq:con_lm_tabular_ni}
%     & \mathbf{n}_i \coloneqq 1 - \prod_k (1- \mathbf{m}_{i,k}), \forall i \in 
%     \{1, \dots, q\}, \\
%     \label{eq:con_lm_tabular_Ni}
%     & \mathbf{N}_i \coloneqq 1 - \prod_k (1- \mathbf{M}_{i,k}), \forall i \in 
%     \{1, \dots, q\}.
% \end{eqnarray}
% Notice that Eq. (\ref{eq:obj_gm_tabular_Ni}), Eq. (\ref{eq:con_lm_tabular_ni}) and Eq. (\ref{eq:con_lm_tabular_Ni}) are not ``real" constraints since both $\mathbf{N}$ and $\mathbf{n}$ are not variables to be optimized, 
% but are intermediate variables computed using $\mathbf{M}$ and $\mathbf{m}$, respectively.


\subsection{Optimization for graphs}
\label{sec:opt_graph}
% We adapt the two-stage optimization framework to extract salient subgraphs~\cite{Yoshida2019kdd} to explain SN prediction on graphs.
Isolated single-edged subgraphs are not only difficult for domain experts to interpret, but can also disturb the working of the GNN within the SN.
Therefore, the selection of two adjacent edges should be related.
% This constraint can be enforced in the first stage.
In stage 1, 
% during the optimization of the global invariant explanation for each graph $G$,
% we add to optimization problem Eq. (\ref{eq:obj_gm})
% a constraint over each pair of adjacent edges that share one node,
we add constraints to optimization problem Eq. (\ref{eq:obj_gm}) to encourage the connectivities,
\begin{align}
% \label{eq:con_lm_obj_graph}
    \min_{\mathbf{M}\in[0,1]^p} &
    \ell \left(
    f(\mathbf{x}, \mathbf{x}),
    f(\mathbf{x}, \mathbf{M} \otimes \mathbf{x})
    \right) 
    + \gamma \| \mathbf{M} \|
    \label{eq:obj_gm_graph}\\
    \textnormal{s.t.} \quad &
    g_{jk}(\mathbf{M}) = \| \mathbf{M}_j - \mathbf{M}_k \| - \epsilon \leq 0,j,k\textnormal{ adjacent in }G. \label{eq:con_gm_graph_connect}
\end{align}
The constraints indicate that the selection of the $j$-th edge can lead to the selection of the $k$-th edge if they share a node~\cite{luo2020parameterized},
where the hyperparameter $\epsilon$ controls the likelihood of two adjacent edges together.
After obtaining $\mathbf{M}$ for each graph,
the local masks of the query graph $\mathbf{G}^s$ and reference graph $\mathbf{G}^t$ are optimized by solving problem Eqs. (\ref{eq:con_lm_obj})-(\ref{eq:con_lm_con_2}), 
with constraints due to the global invariant masks $\mathbf{M}^s$ and $\mathbf{M}^t$.
% \begin{equation}
% \begin{align}
% \label{eq:con_lm_obj_graph}
%     \min_{\mathbf{m}^s, \mathbf{m}^t} 
%     \ell & \left( 
%     f(\mathbf{x}^s, \mathbf{x}^t),
%     f(\mathbf{m}^s \otimes \mathbf{x}^s, 
%     \mathbf{m}^t \otimes \mathbf{x}^t)
%     \right) 
%     + \gamma \left(\| \mathbf{m}^s \| + \| \mathbf{m}^t \| \right),\\
%     \label{eq:con_lm_con_graph_ms}
%     \textnormal{s.t.} \quad &
%     g_i(\mathbf{m}) = \mathbf{m}^s_i - \mathbf{M}^s_i \leq 0, 
%     \forall i \in \{1, \dots, p_s\}, \\
%     & \label{eq:con_lm_con_graph_mt}
%     g_{p_s+i}(\mathbf{m})=
%     \mathbf{m}^t_i - \mathbf{M}^t_i \leq 0, 
%     \forall i \in \{1, \dots, p_t\}.
    % &
    % g_{jk}(\mathbf{m}^s) = \| \mathbf{m}_j^s - \mathbf{m}_k^s \| - \epsilon \leq 0,j,k\textnormal{ adjacent in }G^s, \label{eq:con_lm_con_graph_connect_gs}\\
    % & g_{uv}(\mathbf{m}^t) = \| \mathbf{m}_u^s - \mathbf{m}_v^s \| - \epsilon \leq 0,u,v\textnormal{ adjacent in }G^t. \label{eq:con_lm_con_graph_connect_gt}
% \end{align}
% Due to the flexibility of graphs,
In general, $\mathbf{G}^s$ and $\mathbf{G}^t$ have different numbers of nodes, 
thus $\mathbf{x}^s$ and $\mathbf{x}^t$
(accordingly, $\mathbf{m}^s$ and $\mathbf{m}^t$) can have different dimensions.
% Alternatively, 
Similar to Eq. (\ref{eq:kl_reg}),
we can formulate an unconstrained optimization problem by 
% removing the two sets of inequality constraints and adding two KL regularization terms 
removing constraints and adding KL terms 
$\beta [\textnormal{KL}(\mathbf{m}^s \| \mathbf{M}^s)
+
\textnormal{KL}(\mathbf{m}^t \| \mathbf{M}^t)]$ to the objective.
% similar to Eq. (\ref{eq:kl_reg}).


\subsection{Optimization algorithm and convergence}
% Searching for a global mask $\mathbf{M}$ using
% Eq. (\ref{eq:obj_gm})
% or Eq. (\ref{eq:obj_gm_tabular})
% can be done by off-the-shelf unconstrained optimization solvers.
% Eq. (\ref{eq:con_lm_tabular_obj})
% and Eq. (\ref{eq:con_lm_obj_graph}) are constrained optimization problems and requires some care.
If we adopt the KL-regularization to incorporate global invariance (see Eq. (\ref{eq:kl_reg})),
SGD can be used and
the global masks act as regularization rather than hard constraints.
Alternatively,
local explanations on tabular data (Eq. (\ref{eq:con_lm_tabular_obj})-(\ref{eq:con_lm_tabular_Mi}))
and global/local explanations on graph data (Eqs. (\ref{eq:con_lm_obj})-(\ref{eq:con_lm_con_2}),
or Eqs. (\ref{eq:obj_gm_graph})-(\ref{eq:con_gm_graph_connect})) can be found by solving constrained optimization problems.
However, the constraints should not be hard constraints: two adjacent edges do not have to be always selected simultaneously, and a local mask can select features outside the global explanations to accommodate different references (see Figure~\ref{fig:mask_demon}).
% We turn the inequality constraints to soft constraints.
Slack variables can help as in soft-SVM~\cite{bishop2006pattern} but introduce more primal and dual variables and hyperparameters.
% One way is to introduce a non-negative slack variable to each inequality constraint and add the sum of the slack variables to the objective functions.
% This approach has two drawbacks: first, the reformulation makes the problem more complex with additional variables and constraints (non-negativity of the slack variables), and second, the relative importance between the sum of slack variables and other terms in the objective function needs an additional hyperparameter that itself needs to be optimized.

We adopt a gradient descent-ascent (GDA) in algorithm~\cite{cotter2019optimization} to allow violations of the constraints.
Take optimizing local masks as an example,
the mask to optimize is
$\mathbf{m}=\mathbf{m}^s=\mathbf{m}^t$ for tabular data
and $\mathbf{m} = [\mathbf{m}^s; \mathbf{m^t}]$ (the concatenation of $\mathbf{m}^s$ and  $\mathbf{m^t}$) for graph data.
The objective function $g_0(\mathbf{m})$ is that in Eq. (\ref{eq:con_lm_obj}) or Eq. (\ref{eq:con_lm_tabular_obj}),
and the inequality constraints $g_i(\mathbf{m}), \forall i \in \{1, \dots, c \}$ are those defined in Eqs. (\ref{eq:con_lm_con_1})-(\ref{eq:con_lm_con_2}) or Eq. (\ref{eq:con_lm_tabular_ineq}),
with $c$ being the total number of inequality constraints in each problem.
%the number of major features for tabular data,
% and $c=p_s+p_t$ for graph data.
% Given an objective function $g_0(\mathbf{m})$ and $c$ constraints 
% $g_i(\mathbf{m}), \forall i \in \{1,\dots,c\}$,
We introduce the non-negative Lagrange multipliers $\boldsymbol{\lambda}  \in\mathbb{R}_+^{c}$
and construct the Lagrangian
\begin{equation}
\label{eq:lagrangian}
\mathcal{L}(\mathbf{m}, \boldsymbol{\lambda}) 
= g_0(\mathbf{m}) + \sum_{i=1}^{c} \lambda_i g_i(\mathbf{m}),
\end{equation}
The partial derivatives of $\mathcal{L}$ with respect to $\mathbf{m}$ and $\boldsymbol{\lambda} $ are
\begin{equation}
\label{eq:gradient_lag}
    \frac{\partial \mathcal{L}}{\partial \mathbf{m}} = 
    \frac{\partial g_0}{\partial \mathbf{m}} + \sum_{i=1}^{c} \lambda_i \frac{\partial g_i}{\partial \mathbf{m}}, \hspace{.2in}
    % g_1^\prime(lm) + \sum_{i=2}^{c+1} \boldsymbol{\lambda}_i g_i^\prime(lm), \\
    \frac{\partial \mathcal{L}}{\partial {\boldsymbol{\lambda}}} = \left[g_1(\mathbf{m}), \dots, g_c(\mathbf{m})\right].
    % \quad
    % \frac{\partial \mathcal{L}}{\partial \lambda_i} = , i =1,\dots, c.
\end{equation}
Then gradient descent is applied to $\mathbf{m}$ and gradient ascent is applied to $\boldsymbol{\lambda}$ with learning rates $\eta_1$ and $\eta_2$:
\begin{equation}
\label{eq:variable_update}
    \mathbf{m} \leftarrow \mathbf{m} - \eta_1  
    \frac{\partial \mathcal{L}}{\partial \mathbf{m}},
    \hspace{.2in}
    \boldsymbol{\lambda} \leftarrow \boldsymbol{\lambda} + \eta_2 
    \frac{\partial \mathcal{L}}{\partial \mathbf{\boldsymbol{\lambda}}}.
\end{equation}
Between the two updates, we use the latest $\mathbf{m}$ to evaluate the partial derivatives with respect to  $\boldsymbol{\lambda}$.
Also, the $\boldsymbol{\lambda}$ vector is normalized to have length one before entering the next update iteration.
The GDA-based SN explanation (SNX) algorithm is given in Algorithm~\ref{alg:con_opt}.
% where $\frac{\partial g_0}{\partial \mathbf{m}}$ is the first order partial derivative.
% Algorithm \ref{alg:con_opt} shows the GDA to find the global and local masks for $\mathbf{x}^s$ and $\mathbf{x}^t$,
% alternatively applying gradient descent to $\mathbf{m}$ and gradient ascent to $\boldsymbol{\lambda}$.
% We refer to the GDA that find local masks with global invariant constraint as SNX,
If an unconstrained KL-regularized optimization problem is solved for the local masks,
we refer to the algorithm as SNX-KL.
% To fit the tabular data,
% one can set $\mathbf{m}^s=\mathbf{m}^t$,
% and apply the objective functions and constraints specified in Eq. (\ref{eq:obj_gm_tabular}) to Line 4 for extracting global masks
% and Eq. (\ref{eq:con_lm_tabular_con}) to Line 8 for local ones.
% As for the graph data,
% one can specify Eq. (\ref{eq:obj_gm_graph}) to Line 4 and Eq. (\ref{eq:con_lm_con_graph}) to Line 8.

\begin{algorithm}[t]
\caption{SNX: Siamese Network Explanation with GDA}
\label{alg:con_opt}
\begin{algorithmic}[1]
\STATE \textbf{Input}: 
a target SN model $f$, 
a query instance $\mathbf{x}^s$ and reference instance $\mathbf{x}^t$,
\textit{optional} human-defined constraints in $\mathbf{M}^s$ and $\mathbf{M}^t$,
learning rate $\eta_1, \eta_2$ for $\mathbf{m}$ and $\boldsymbol{\lambda}$.
\STATE \textbf{Output}:
% local masks $\mathbf{m}^s$ and $\mathbf{m}^t$ for $\mathbf{x}^s$ and $\mathbf{x}^t$, respectively.
local masks $\mathbf{m}^s$ for $\mathbf{x}^s$, and $\mathbf{m}^t$ for $\mathbf{x}^t$.
\STATE \textbf{Init}:
$\boldsymbol{\lambda} = [1/c,\dots,1/c]\in\mathbb{R}^{c}$.
\IF{$\mathbf{M}^s$ and $\mathbf{M}^t$ not given}
\STATE Extract global masks $\mathbf{M}^s$ and $\mathbf{M}^t$ by 
Eqs. (\ref{eq:obj_gm_tabular})-(\ref{eq:obj_gm_tabular_Ni}) (for tabular data) 
or 
Eqs. (\ref{eq:obj_gm_graph})-(\ref{eq:con_gm_graph_connect}) (for graph).
% \hfill{$\rhd$Self-supervised.}
\hfill{$\rhd$SSL}
\ENDIF
\STATE Pretrain local masks $\mathbf{m}^{s}, \mathbf{m}^t$ without constraints using Eqs. (\ref{eq:con_lm_tabular_obj}) and (\ref{eq:con_lm_tabular_mi}) (for tabular data) or  Eq. (\ref{eq:con_lm_obj}) (for graph).
\STATE Solve the full constrained optimization problems Eqs. (\ref{eq:con_lm_tabular_obj})-(\ref{eq:con_lm_tabular_Mi}) (tabular) or Eqs. (\ref{eq:con_lm_obj})-(\ref{eq:con_lm_con_2}) (graph) using GDA to find $\mathbf{m}^s$ and $\mathbf{m}^t$.
% \STATE Solve the KL-regularized unconstrained problem to find $\mathbf{m}^s$ and $\mathbf{m}^t$.
% \FOR {$iter = 1 \to  MaxIter$}
%     \STATE Update $\mathbf{m} \leftarrow \mathbf{m} - \eta_1 * 
%     \frac{\partial \mathcal{L}}{\partial \mathbf{m}} $
%     % \Delta_{\mathbf{m}}$ 
%     by Eq. (\ref{eq:gradient_lag})
%     for $\mathbf{m}^s$ and $\mathbf{m}^t$;
%     \STATE Recompute constraints with the updated $\mathbf{m}$ by
%     Eq. (\ref{eq:con_lm_tabular_ineq});
%     \STATE Update $\boldsymbol{\lambda} \leftarrow \boldsymbol{\lambda} + \eta_2 *
%     \frac{\partial \mathcal{L}}{\partial \mathbf{\boldsymbol{\lambda}}} $
%     % \Delta_{\boldsymbol{\lambda} }$ 
%     by Eq. (\ref{eq:gradient_lag});
%     \STATE Normalize $\boldsymbol{\lambda} \leftarrow \boldsymbol{\lambda} / \| \boldsymbol{\lambda} \|$.
%     % \STATE Extract $lm$ with constraints by Eq. (\ref{eq:obj_lm})
%     % \STATE constrains = hinge(0, $lm - gm$) \in \mathbb{R}^c
% \ENDFOR
\end{algorithmic}
\end{algorithm}

\noindent\textbf{Convergence}.
The Lagrangian is nonconvex-concave, in fact, linear in the dual variables.
The GDA algorithm is convergent based on Theorem 4.4 of the work~\cite{lin20a}, given the Lagrangian satisfies their Assumption 4.2, reproduced below:

\begin{enumerate}[leftmargin=*]
    \item 
\textit{ $\mathcal{L}$ is $l$-smooth and $\mathcal{L}(\cdot,\boldsymbol{\lambda})$ is $L$-Lipschitz for each $\boldsymbol{\lambda}$ and $\mathcal{L}(\mathbf{m},\cdot)$ is concave for each $\mathbf{m}$.
}
    \item
\textit{The domain of $\boldsymbol{\lambda}$ is convex and bounded.}
\end{enumerate}

We verify these assumptions:
if the target SN is a composition of smooth function (excluding functions such as ReLU), then $\mathcal{L}$ is smooth in both the primal variable $\mathbf{m}$ and the dual variable $\boldsymbol{\lambda}$;
% The $\ell 1$ penalties on the masks are not an issue 
since the masks are all non-negative, the $\ell 1$ penalties turn out to be just the sum of the elements in the masks.
Due to the smoothness, $\mathcal{L}(\cdot,\boldsymbol{\lambda})$ is $L$-Lipschitz. %, though the constant $L$ is hard to estimate in general.
$\mathcal{L}$ is linear and thus concave in $\boldsymbol{\lambda}$.
In Algorithm~\ref{alg:con_opt}, we normalize $\boldsymbol{\lambda}$ to the unit ball and thus the second assumption is satisfied.






% \subsection{Decoding for explanations}
% \label{sec:decoding}
% In some explanation methods, 
% like those using attention models \cite{serrano2019attention},
% the salient features are highlighted by the attention weights. 
% Some other explanations select the top important features as explanations, 
% while discarding the remaining ones. 
% Decoding means post-processing the optimal masks to obtain final explanations that satisfy constraints, such as graph connectivity or feature value monotonicity~\cite{mothilal2020explaining}, that are non-convex or non-differentiable to be incorporate in explanation optimization.

% For tabular data, 
% it is like a feature selection algorithm: 
% one can simply select the features with the highest mask values. 
% For graphs, 
% the situation is more complex.
% Depending on what the end-users want, 
% subgraphs of various sizes and connectivity can be extracted. 
% If one does not care about the graph structure, 
% then the selection is the same as the tabular data case. 
% If larger connected subgraphs are desired, 
% we propose to use a spanning tree algorithm to decode the masks for the final subgraphs. 

% \begin{algorithm}[t]
% \caption{Graph decoding by the spanning tree.}
% \label{alg:graph_decoding}
% \begin{algorithmic}[1]
% \STATE \textbf{Input}: 
% A mask $\mathbf{m}$ from Eq. (\ref{eq:con_lm_obj_graph}), 
% and a $ratio$ of selected edge.
% \STATE \textbf{Output}:
% A spanning tree $\mathbf{m}^\prime$ generated by $\mathbf{m}$.
% \STATE \textbf{Init}:
% $\mathbf{m}^\prime = \mathbf{I}_{|V|\times|V|}$,
% % TreeNode = $list()$.
% \STATE 
% Sort $\mathbf{m}$ by its value and record the original location $loc$.
% \STATE 
% % $a = \mathbf{m}.\texttt{pop}(0)$, 
% $ (i,j) = loc.\texttt{pop}(0)$;
% % \STATE 
% $\mathbf{m}^\prime[i][j]= \mathbf{m}^\prime[j][i] =1$;
% TreeNode = $[i, j]$
% \WHILE{TreeNode.size $- 1 \leq ratio * |E|$}
% % \FOR{$(i,j) \in loc$}
% \FOR{$idx = 0 \to loc$.size }
% \STATE $(i,j) = loc[idx]$
% \IF{$i \in$ TreeNode \textbf{OR} $j \in$ TreeNode } 
% \STATE 
% $loc.\texttt{pop}(idx)$;
% $\mathbf{m}^\prime[i][j]= \mathbf{m}^\prime[j][i] =1$;
% \STATE
% TreeNode.\texttt{push}($i$);
% TreeNode.\texttt{push}($j$)
% \ENDIF
% \ENDFOR
% \ENDWHILE
% % \WHILE{TreeNode-1}
% % \STATE a
% % \ENDWHILE
% \end{algorithmic}
% \end{algorithm}




==> yifan.tex <==
\section{Yifan}
\subsection{Data and Related work}
\noindent\textbf{Data}.
Given an dataset contains $n$ graphs, e.g., $\mathcal{G}=\{G_1,G_2,\dots,G_n\}$,
each of which has different edges $E$ and nodes $V$,
we use d-dimensional node features $\mathcal{X}=\{X_1,X_2,\dots,X_m\},X\in\mathbb{R}^d$, 
to represent all the nodes,
and use binary adjacency matrix $A(G)=\{0,1\}^{m\times m}$, 
to describe the graph structure.

\noindent\textbf{Siamese Network}.
A Siamese Network (SN) takes two samples as input and outputs their similarity indicating how likely two samples are from the same class. 

Here, we apply $SN$ to Graph Convolutional Network (GCN).
Formally, given two samples $G_i', G_j'$,
each has node feature $\mathcal{X}$ and adjacency matrix $A(G)$.
Siamese GCN trains a n-dimensional vector for every sample and based on the vector distance,provides a higher score (closer to 1) for pairs from the same class and lower score (closer to 0) for different-class pairs.$SN(G_i,G_j) = score_{i,j}$,$EMB(G_i) = embedding_i$

In the rest of this section, 
we assume that the Siamese Network has been trained well and \textit{fixed} for explanation.

\noindent\textbf{GNNExplainer}.
For Graph Neural Networks (GNNs), GNNExplainer can generate consistent and concise explanations for nodes and graphs.

Here, we use GNNExplainer to generate a explaination for a single graph as we only provide GCN model which has been trained well for graph classification.

\subsection{Objective function}
\noindent\textbf{Motivation}.
Differing from GNNExplainer, Siamese Network takes two inputs into account at the same time. 
Explanation should consider two inputs together as well.
Motivated by it, we propose a two-step explanation.
In the first step, we want to provide a local explaination by considering two graph at the same time. So the explaination can provide a more personalized explanation for the two samples.
In the second step, in order to get more general explantiaon, we fix one sample and match with multiple samples to get multiple local explanations about a sample. Then by the approximate calculation of the largest common subgraph in local explainations, we can find a global explaination for the fixed sample which keeps consistency in specific interpretation.

\noindent\textbf{Objective functions}.
To extract the ``local" features, we optimize the mask (node selector) by 

siameselabel =
$\begin{cases}
1, & \mbox{if } SN(G_i,G_j) \mbox{ $\geq   0.5$} \\
0, & \mbox{if } SN(G_i,G_j) \mbox{ $< 0.5$}
\end{cases}
$

\begin{equation}
\begin{aligned}
    \min_{lm_i,lm_j} \textnormal{BCE} \{ SN(G_i\otimes lm_i, G_j\otimes lm_j)), siameselabel \} \\
    + \lambda ||lm_i||+\lambda  ||lm_j||,\\
     s.t.  \quad lm_i \leq A(G_i), \quad i=\{1,2,\dots,p\} \\
\end{aligned}
\end{equation}
where BCE($x,label$) = $-(label\log(x) + (1-label)\log(1-x) )$ is the Binary Cross Entropy,
$||lm||$ is the $\ell$1-norm of the mask,
$\otimes$ is the Hadamard (element-wise) product, and $\lambda$ is hyper-parameter controlling the sparsity of $lm$.
Ideally, $lm$ extracts the most ``informative" nodes which keeps the different of $G_i$ and $G_j$after masks as closed to original $G_i'$ as possible.

The largest common subset problem is an NP-hard problem. So in order to find the ``global" mask, we use heuristic algorithms to find the most suitable common subgraph among the ``local" mask.



Datasets and model structure
\noindent \textbf{Datasets.}
\textcolor{blue}{For graph data}
we conduct experiments on two datasets as shown in Table \ref{tab:datasets}. 
{molecule} is used to predict if the molecule is protein or not.
\textbf{brain} is used to predict if a person will subscribe a term deposit.

We spilt the instances into training set and test set with the ratio of $60:40$.
For the inference,
we randomly select two positive-class and negtive-class instances,
respectively, 
for each instance in both training and test portions.
For the explanations,
all the instances are from test portion.
We randomly select 100 references from positive-class and negtive-class to constitute 20000 pairs same-class instances and 10000 pairs different-class instances.

\noindent \textbf{Structures of the target SN model.}
For tabular data,
the target SN model utilizes an MLP layer as the mapping function $emb(\mathbf{x};\theta) = \theta_1^\top\mathbf{x}$ + $\theta_0$,
the cosine-similarity as the similarity function,
and the hinge loss as training loss function 
$\ell^{SN} = \textnormal{max}\{0, 1-y_{st}*f(\mathbf{x}^s, \mathbf{x}^t; \theta) \}$.

\textcolor{blue}{For graph data}
the target SN model utilizes two graph convolution layer and a mean-pooling layer as the mapping function and 
the  euclidean\_distance as the similarity function,
and the hinge loss as training loss function 
$\ell^{SN} = \textnormal{max}\{0, 4-y_{st}*f(\mathbf{x}^s, \mathbf{x}^t; \theta) \}$.



\subsection{Baselines}
For both tabular data and graph data,
we compare our methods with the following baselines and group them depending on whether generating global $\mathbf{M}$ and local masks $\mathbf{m}$. 
We remark if one is specific for tabular data or graph data.

\noindent \textbf{Extracting global masks}.
\begin{itemize}[leftmargin=*]
    \item \textit{Pick-all} set all elements in the masks to one,
    and \textit{Pick-none} set all elements to zero, 
    both of which provide ``upper-bound'' and ``lower-bound'' when evaluating other methods.
    \item \textit{DES-global} \cite{wei2017rethinking} provides a state-of-the-art method to score the importance of features in unsupervised classification tasks without consideration of SN structure.
    It generates the pseudo labels for all pairs of instances by kNN, 
    and learning a NN based on the pseudo labels.
    It does not generate customized explanations for each pair but general explanations for all pairs.
    (Tabular data only)
    \item As mentioned in Sec. \ref{sec:opt_tabular},
    we explore the performance of two variants of XX for global masks,  
    $\mathbf{M}_i = \min (\mathbf{M}^s_i, \mathbf{M}^t_i)$ and
    $\mathbf{M}_i=\max (\mathbf{M}^s_i,  \mathbf{M}^t_i)$,
    denoted as \textit{XX-inter} and \textit{XX-union}, respectively.
    (Tabular data only)
\end{itemize}

\noindent \textbf{Extracting local masks}.
\begin{itemize}[leftmargin=*]
    \item \textit{Pick-all} and \textit{Pick-none} are used for the same purpose.
    \item \textit{Gradient-based} \cite{baldassarre2019explainability} finds the features with largest gradients as salient features.
    \item
    \textit{DES-global} uses the importance scores as the local masks directly.
    (Tabular data only)
    \item \textit{XX-global} uses global masks by Eq. (\ref{eq:obj_gm_tabular}) for tabular data and Eq. (\ref{eq:obj_gm_graph}) for graph data directly without further searching for local masks,
    such that $\mathbf{m}^s=\mathbf{M}^s$ and $\mathbf{m}^t=\mathbf{M}^t$.
    \item
    \textit{KL-soft} considers the constraints $P\leq Q$ by putting $KL(P\|Q)$ into the objective function \cite{bishop2006pattern},
    which provides soft-constraints.
    \item \textit{Unconstrained-local} solves the unconstrained optimization in Eq. (\ref{eq:obj_lm}) without considering any constraints.
    \item
    \textit{DES-local} optimizes $\mathbf{m}$ by Eq. (\ref{eq:con_lm_tabular_obj}) and Eq. (\ref{eq:con_lm_tabular_con}) where $\mathbf{M}$ is provided by \textit{DES-global}.
    (Tabular data only)
    \item \textit{XX-inter} and \textit{XX-union} optimizes $\mathbf{m}$ based on their global masks mentioned previously.
    (Tabular data only)
\end{itemize}
